Sparse Kalman Filtering Approaches to Covariance Estimation from High Frequency Data in the Presence of Jumps

Estimation of the covariance matrix of asset returns from high frequency data is complicated by asynchronous returns, market mi- crostructure noise and jumps. One technique for addressing both asynchronous returns and market microstructure is the Kalman-EM (KEM) algorithm. However the KEM approach assumes log-normal prices and does not address jumps in the return process which can corrupt estimation of the covariance matrix. In this paper we extend the KEM algorithm to price models that include jumps. We propose two sparse Kalman filtering approaches to this problem. In the first approach we develop a Kalman Expectation Conditional Maximization (KECM) algorithm to determine the un- known covariance as well as detecting the jumps. For this algorithm we consider Laplace and the spike and slab jump models, both of which promote sparse estimates of the jumps. In the second method we take a Bayesian approach and use Gibbs sampling to sample from the posterior distribution of the covariance matrix under the spike and slab jump model. Numerical results using simulated data show that each of these approaches provide for improved covariance estima- tion relative to the KEM method in a variety of settings where jumps occur.

==> SecECM_v6.tex <==
\section{KECM Approach to estimation of $\Gamma$}
\label{Sec:ECM}
Maximum a posteriori (MAP) estimation of $\Gamma$ is examined in this section.  The MAP estimate is defined as the conditional mode of the posterior log-likelihood.
There are several approaches to determining MAP estimates such as gradient ascent and Newton's method.   However, computation of the gradients and Hessian required for these techniques can make these intractable for large problems.   For this problem determining the MAP estimate is a non-concave maximization problem and thus our MAP estimates may only be locally optimal.

In this section we propose two Kalman ECM (KECM) techniques for determining a MAP estimate of $\Gamma$.  The benefit of this approach is that each iteration can be performed without computing derivatives.   The first ECM approach is an approximate technique where the prior distribution on the jumps is approximated as a Laplace distribution.  The advantage of this approximation is that the conditional maximization steps in the ECM algorithm are concave maximization problems for which global (conditional) optimal solutions can be obtained.
The disadvantage is that we are approximating the true spike and slab jump model.   The second approach uses the spike and slab model for jumps, which is a true representation of the model presented in Section \ref{Sec:ModelHigh}.   However we will see that using the spike and slab jump model results in a non-concave optimization problem in the conditional M-step for $J$.

%In this section we address the problem of obtaining a maximum a posteriori (MAP) estimate of $\Gamma$.   The posterior log-likelihood given the complete data $(X,Y)$ can be easily derived using the relations in Section %\ref{Sec:ModelHigh}.   However the problem is complicated by the fact that $X$ is unobserved.   Thus we must marginalize out $X$ in the complete data model to obtain the posterior log-likelihood given $Y$.   This involves an %intractable multi-dimensional integral.

%A more tractable approach to determining a MAP estimate of $\Gamma$ is to use the Expectation-Maximization (EM) algorithm CITE(RUBIN).  This problem was considered for cases without jumps in SHUMWAY,OTHER.   Extending this %approach ................

%Recall the previous section the jump model is equivalent to a switching state space model.   Inference in switching state space models becomes intractable as the number of states increase \cite{Ghahramani}.   For example %estimation of the posterior distribution of $X$ given $Y$ involves marginalizing out the $2^{TN-N}$ possible states for $Z$, which is an intractable integral.   Maximum a posteriori (MAP) estimation of $Z$ is also difficult due %to the multi-model nature of $p(z)$.

%Since the log-posterior for our model is non-concave obtaining a MAP estimate is a difficult optimization problem.
%In this section we propose a Kalman-ECM (KECM) approach to determining a maximum a posteriori (MAP) estimate of $\Gamma$.   The KECM approach breaks





%Considering these difficulties we propose an approximate approach for estimation of $\Gamma$.  In our approximation we relax the prior distribution on the jumps to a continuous distribution.   This approximation is then used to %derive ECM \cite{ECMRubin} approach for determining $\Gamma$.
%\input{SubSecEM}



\subsection{KECM algorithm for Laplace Distribution}
First we consider a KECM approach to estimating $\Gamma$ when $J_{i}$ is approximated by a Laplace distributed random variable.  We define
\begin{equation*}
\Theta = [\Theta_{1},\Theta_{2},\Theta_{3},\Theta_{4},\Theta_{5}]
\end{equation*}
where
\begin{eqnarray*}
% \nonumber to remove numbering (before each equation)
\Theta_{1} &=& D  \\
\Theta_{2} &=& \Gamma \\
\Theta_{3} &=& \sigma_{o}^{2}  \\
\Theta_{4} &=& J(2:T) \\
\Theta_{5} &=& \lamSetInv
\end{eqnarray*}
as our vector of unknown parameters and $X(1:T)$ as the latent variables.

The KECM approach is an iterative algorithm that can be applied to the following problem
\begin{equation*}
  \Theta^{*} = \arg\max_{\theta} L(\theta)
\end{equation*}
where $L(\theta)$ is the log posterior of $\Theta$.   In the KECM algorithm we iterate over E-steps and conditional M-steps to arrive at an estimate of $\Theta$.

The E-step in the KECM algorithm involves computing the expected value of
\begin{equation*}
  \log p(X(1:T),y(1:T)|\theta)p(\theta)
\end{equation*}
with respect to $p(x(1:T)|y,\Theta^{(k)})$
\begin{equation*}
  \mathcal{G}(\theta,\Theta^{(k)}) = \mathbb{E}_{p(x|y,\Theta^{(k)})}\log p(X(1:T),y(1:T)|\theta)+\log(p(\theta))
\end{equation*}
where $\Theta^{(k)}$ is an estimate of $\Theta$ at the $k^{th}$ iteration and where $p(\theta)$ is the prior distribution of parameters
\begin{equation*}
p(\theta)=p(\theta_{1})p(\theta_{2})p(\theta_{3})g(\theta_{4},|\lambda)q_{inv}(\lambda^{-1}).
\end{equation*}
Here the complete log-likelihood is
\begin{eqnarray*}
  \log p(x,y|\theta) &=& -M \log(\sigma) -\frac{1}{2\sigma^{2}}\sum_{t=1}^{T}||y(t)-\tilde{I}(t)x(t)||_{\ell_{2}}^{2} \nonumber \\
   && - \frac{T-1}{2}\log(|\Gamma|) \nonumber \\
   && - \frac{1}{2}\sum_{t=2}^{T}r(t)^{T}\Gamma^{-1}r(t) \nonumber \\
   && + const
\end{eqnarray*}
where $M$ is the total number of observed asset prices and where
\begin{equation*}
   r(t)=x(t)-x(t-1)-d-j(t).
\end{equation*}





The EM approach prescribes a joint maximization of $\mathcal{G}(\theta,\Theta^{(k)})$  with respect to $\theta$.   This is difficult due to the coupling of variables and the non-concavity of the problem.   Thus we apply conditional maximization as in the ECM \cite{ECMRubin} or coordinate ascent algorithm.   The conditional M-steps involves a coordinate-wise maximization of $\mathcal{G}$.  Here the conditional M-steps are
\begin{eqnarray}
  \Theta_{1}^{(k+1)} = \arg\max_{\theta_{1}} \mathcal{G}\left(\left[\theta_{1},\Theta_{2}^{(k)},\Theta_{3}^{(k)},\Theta_{4}^{(k)},\Theta_{5}^{(k)} \right],\Theta^{(k)}\right) \nonumber \\
  \Theta_{2}^{(k+1)} = \arg\max_{\theta_{2}} \mathcal{G}\left(\left[\Theta_{1}^{(k+1)},\theta_{2},\Theta_{3}^{(k)},\Theta_{4}^{(k)},\Theta_{5}^{(k)}\right],\Theta^{(k)}\right) \nonumber \\
  \Theta_{3}^{(k+1)} = \arg\max_{\theta_{3}} \mathcal{G}\left(\left[\Theta_{1}^{(k+1)},\Theta_{2}^{(k+1)},\theta_{3},\Theta_{4}^{(k)},\Theta_{5}^{(k)}\right],\Theta^{(k)}\right) \nonumber \\
  \Theta_{4}^{(k+1)} = \arg\max_{\theta_{4}} \mathcal{G}\left(\left[\Theta_{1}^{(k+1)},\Theta_{2}^{(k+1)},\Theta_{3}^{(k+1)},\theta_{4},\Theta_{5}^{(k)}\right],\Theta^{(k)}\right) \nonumber \\
  \Theta_{5}^{(k+1)} = \arg\max_{\theta_{5}} \mathcal{G}\left(\left[\Theta_{1}^{(k+1)},\Theta_{2}^{(k+1)},\Theta_{3}^{(k+1)},\Theta_{4}^{(k+1)},\theta_{5}\right],\Theta^{(k)}\right).  \label{eqTheta3}
\end{eqnarray}
Each of these problems is a concave optimization problem which can be readily solved.
\subsubsection{E-step of KECM}
%The complete log-posterior distribution $\log(p(x|y,\theta))$ separates into terms involving only $\lambda$ and only $x$ which simplifies the calculation.   The term involving only $\lambda$ is
%\begin{equation}\label{eq:LamOnlyTerm}
%  - \lambda\sum_{t=2}^{T}||j(t)||_{\ell_{1}} + const
%\end{equation}
%where $const$ is a term not involving $\theta$.   Taking the expectation of \eqref{eq:LamOnlyTerm} with respect to $p(x,\lambda|y,\theta)$ can be computed as
%\begin{equation}\label{eq:LamOnlyTermMean}
%   - \sum_{t=2}^{T}||j(t)||_{\ell_{1}}\left(\frac{\frac{1}{M_{\lambda}}\sum_{i=1}^{M_{\lambda}}\tilde{\lambda_{i}}\tilde{\lambda}_{i}^{(T-1)N}\exp(-\tilde{\lambda}_{i} \sum_{t=2}^{T}||j(t)||_{\ell_{1}})}{\frac{1}{M_{\lambda}}\sum_{i=1}^{M_{\lambda}}\tilde{\lambda}_{i}^{(T-1)N}\exp(-\tilde{\lambda}_{i} \sum_{t=2}^{T}||j(t)||_{\ell_{1}})}\right) + const
%\end{equation}
%Thus the effect of the E-step for \eqref{eq:LamOnlyTerm} is to replace $\lambda$ with it's posterior mean
%\begin{equation}\label{eq:BarLambda}
%  \bar{\lambda}=\left(\frac{\frac{1}{M_{\lambda}}\sum_{i=1}^{M_{\lambda}}\tilde{\lambda_{i}}\tilde{\lambda}_{i}^{(T-1)N}\exp(-\tilde{\lambda}_{i} \sum_{t=2}^{T}||j(t)||_{\ell_{1}})}{\frac{1}{M_{\lambda}}\sum_{i=1}^{M_{\lambda}}\tilde{\lambda}_{i}^{(T-1)N}\exp(-\tilde{\lambda}_{i} \sum_{t=2}^{T}||j(t)||_{\ell_{1}})}\right)
%\end{equation}
The posterior $p(x|y,\Theta^{(k)})$ needed to perform the E-step is normal and can be computed using a Kalman smoother \cite{Shumway}.
Since the posterior is normal it is defined completely by the following posterior moments for $m=T$
\begin{equation*}
  \bar{X}(t|m) \doteq \E(X(t)|y(1:m))
\end{equation*}
\begin{equation*}
  P(t|m) \doteq \cov(X(t),X(t)|y(1:m))
\end{equation*}
\begin{equation*}
  P(t,t-1|m) \doteq \cov(X(t),X(t-1)|y(1:m))
\end{equation*}
where $\cov(:,:)$ refers to the covariance function.   Equations for these quantities are derived in \cite{ShumwayBook} and are stated in Appendix \ref{secAppendixSmooth}.
The expected value of log-posterior distribution with respect to the posterior of $X(1:T)$ can be shown to be
\begin{eqnarray}\label{eqPosteriorECM}
  \mathcal{G}(\theta,\Theta^{(k)})&=& \mathbb{E}_{p(x|y,\Theta^{(k)})}\log p(X(1:T),y(1:T)|\theta)+\log(p(\theta)) \nonumber \\
  &=&-\frac{T-1}{2}\log(|\Gamma|) - \frac{1}{2}\textnormal{tr}(\Gamma^{-1}(C-B-B^{T}+A)) \nonumber \\
   & & - M\log(\sigma) \nonumber \\
   && -\frac{1}{2\sigma^{2}}\sum_{t=1}^{T}||y(t)-\tilde{I}(t)\bar{X}(t)||_{\ell_{2}}^{2} + \textnormal{tr}(P(t|T)\tilde{I}(t)^{T}\tilde{I}(t)) \nonumber \\
   && + \log(p(\theta)) + const
\end{eqnarray}
where
\begin{equation*}
  A=\sum_{t=2}^{T} \left(P(t-1|T) + \bar{X}(t-1|T)\bar{X}(t-1|T)^{T} \right)
\end{equation*}
\begin{equation*}
  B=\sum_{t=2}^{T} \left(P(t,t-1|T) + (\bar{X}(t|T)-D^{(k)}-J^{(k)}(t))\bar{X}(t-1|T)^{T} \right)
\end{equation*}
\begin{equation*}
  C=\sum_{t=2}^{T} \left(P(t|T) + (\bar{X}(t|T)-D^{(k)}-J^{(k)}(t))(\bar{X}(t|T)-D^{(k)}-J^{(k)}(t))^{T} \right).
\end{equation*}
These equations are derived in Appendix \ref{secAppendixDerive}.   For notational convenience the dependence of $P(t|m)$ and $P(t,t-1|m)$ on the iteration number has been dropped.

\subsubsection{Conditional M-steps of KECM}
For the conditional M-step it can be shown using standard conjugate prior relationships \cite{FinkConjPrior} that
\begin{equation}\label{driftEM}
  %d^{(j+1)} = \frac{1}{T-1}\sum_{t=2}^{T}\bar{X}(t|T)-\bar{X}(t-1|T)-J^{(j)}(t)
  D^{(k+1)} = F\left ( \frac{1}{\sigma_{D}^2}\bar{D}+ \Gamma^{(k)^{-1}}\sum_{t=2}^{T}\bar{X}(t|T)-\bar{X}(t-1|T)-J^{(k)}(t) \right)
\end{equation}
and
\begin{equation}\label{GammaEM}
  \Gamma^{(k+1)} = \frac{1}{T-1+\eta} \left(A+C^{(k)}-B^{(k)}-B^{(k)T}\right) +\frac{1}{T-1+\eta}W.
\end{equation}
where
\begin{equation*}
  F = \left((T-1)\Gamma^{(k)^{-1}}+\sigma_{D}^{-2}I \right)^{-1}
\end{equation*}
\begin{equation*}
  B^{(k)}=\sum_{t=2}^{T} \left(P(t,t-1|T) + (\bar{X}(t|T)-D^{(k+1)}-J(t)^{(k)})\bar{X}(t-1|T)^{T} \right)
\end{equation*}
and
\begin{eqnarray*}
  C^{(k)}&=& \sum_{t=2}^{T} P(t|T) \\
   &&  + \sum_{t=2}^{T} (\bar{X}(t|T)-D^{(k+1)}-J(t)^{(k)})(\bar{X}(t|T)-D^{(k+1)}-J(t)^{(k)})^{T}.
\end{eqnarray*}

Both terms in $\eqref{GammaEM}$ are positive definite.

The conditional M-step for the observation noise variance is
\begin{equation}\label{obsEM}
  %\sigma_{o}^{2,(j+1)} = \frac{1}{M}\sum_{t=1}^{T}||Y(t)-\tilde{I}(t)\bar{X}(t|T)||_{\ell{2}}^{2} + \trace(P(t|T)\tilde{I}(t)^{T}\tilde{I}(t))
  \sigma_{o}^{2,(k+1)} = \frac{2\beta_{o} + \sum_{t=1}^{T}||y(t)-\tilde{I}(t)\bar{X}(t|T)||_{\ell{2}}^{2} + \trace(P(t|T)\tilde{I}(t)^{T}\tilde{I}(t)) }{2\alpha_{o}+2+M}
\end{equation}
where $M$ is the total number of prices observed.
For each conditional M-step $P(t,T)$, $P(t,t-1|T)$ and $\bar{X}(t|T)$ are evaluated with respect to $p(X(1:T)|Y,\Theta^{(k)})$.

To compute the conditional M-step for $J$ we denote
\begin{eqnarray*}
Q(j) &\doteq& \mathcal{G}([\Gamma^{(k+1)},D^{(k+1)},\sigma_{o}^{2,(k+1)},j,\lamSet^{(k)}],\Theta^{(k)}).
\end{eqnarray*}
Then up to a constant not depending on $j$
\begin{eqnarray*} \
Q(j) &=& - \frac{1}{2} \sum_{t=2}^{T}(\bar{X}(t|T)-j(t)-D^{(k+1)})^{T}( \Gamma^{(k+1)})^{-1}(\bar{X}(t|T)-j(t)-D^{(k+1)})\nonumber \\
      && + \sum_{t=2}^{T} (\bar{X}(t|T)-j(t)-D^{(k+1)})^{T}( \Gamma^{(k+1)})^{-1}\bar{X}(t-1|T) \nonumber \\
      &&+ \log(g(j(2:T)|\lamSet^{(k)})) + const_{1}\\
     &=&  - \frac{1}{2}\sum_{t=2}^{T} (\bar{X}(t|T)-j(t)-D^{(k+1)})^{T}( \Gamma^{(k+1)})^{-1}(\bar{X}(t|T)-j(t)-D^{(k+1)})\nonumber \\
      && + \sum_{t=2}^{T}(\bar{X}(t|T)-j(t)-D^{(k+1)})^{T}( \Gamma^{(k+1)})^{-1}\bar{X}(t-1|T) \nonumber \\
      &&- \sum_{t=2}^{T}\EllnW{j(t)}{\lambda(t)}{1} + const_{2}.
\end{eqnarray*}
where $\EllnW{j(t)}{\lambda(t)}{1} = \sum_{n=1}^{N}\lambda_{n}(t)|j_{n}(t)|$.
By rearranging terms we can express $Q(j)$ as a quadratic function of $j$
\begin{eqnarray*} \
Q(j) &=& - \frac{1}{2} \sum_{t=2}^{T}j(t)^{T}( \Gamma^{(k+1)})^{-1}j(t)\nonumber \\
      && + \sum_{t=2}^{T}(\bar{X}(t|T)-D^{(j+1)}-\bar{X}(t-1|T))^{T}(\Gamma^{(k+1)})^{-1}j(t) \nonumber \\
      &&- \sum_{t=2}^{T}\EllnW{j(t)}{\lambda(t)}{1} + const_{3}.
\end{eqnarray*}

Referring to equation \eqref{eqTheta3} we see that $J^{(k+1)}(t)$ is the solution of the following $\ell_{1}$ penalized quadratic program
\begin{align}\label{eqJumpProb}
J^{(k+1)}(t) =\arg\min_{j} \frac{1}{2}j^{T}( \Gamma^{(k+1)})^{-1} j - j^{T}(\Gamma^{(k+1)})^{-1}\Delta^{(k+1)} + \EllnW{j(t)}{\lambda(t)}{1}
\end{align}
where
\begin{equation} \label{eqJumpLaplaceEM}
  \Delta^{(k)}(t)=\bar{X}(t|T)-D^{(k)}-\bar{X}(t-1|T).
\end{equation}
This problem can be solved with a variety of fast algorithms such as ADMM \cite{ADMM} and FISTA \cite{FISTA}.

Now we determine $\lamSetInv$ which depends only on $q_{inv}(\lambda^{-1})$ and $p(j|\lambda)$.  Using conjugate prior relationships
we have
\begin{equation}\label{eqLamInvUp}
  \lambda_{i}(t)^{-1} = \frac{|J^{(k+1)}_{i}(t)|+\beta_{\lambda}}{\alpha_{\lambda}+2}.
\end{equation}
which implies that
\begin{equation}\label{eqLamUp}
  \lambda_{i}(t) = \frac{\alpha_{\lambda}+2}{|J^{(k+1)}_{i}(t)|+\beta_{\lambda}}.
\end{equation}

An outline of the KECM algorithm for Laplace jump models is given below.
\begin{algorithm}[H]
\caption{KECM Algorithm for estimation of $\Gamma$ under Laplace Prior}
\label{Alg:ECM}
\begin{algorithmic}
\STATE  \textbf{Initialize: }$\Theta^{(0)},k=0$
\WHILE{ not converged}
\STATE Compute $\bar{X}(t|T), P(t|T),P(t,t-1|T)$ using Kalman smoothing equations for $\Theta^{(k)}$  using equations \eqref{eq:ForwardEq}-\eqref{eq:BackwardRecursion}
\STATE Compute $D^{(k+1)},\Gamma^{(k+1)}$, and $\sigma_{o}^{2,(k+1)}$ using equations \eqref{driftEM},\eqref{GammaEM}, and \eqref{obsEM} respectively
\STATE Compute $J^{(k+1)}$ by solving \eqref{eqJumpLaplaceEM}
\STATE Compute $\lamSet$ by solving \eqref{eqLamUp}
\STATE $k=k+1$
\ENDWHILE
\end{algorithmic}
\end{algorithm}
A convergence proof of this algorithm is given in Appendix \ref{Sec:ConvergeECM}.

\begin{remark}
\textnormal{
Since of value of $\lamSet$ changes with each iteration we see that we effectively reweight the $\ell_{1}$ penalty in \eqref{eqJumpProb} after each iteration.   Reweighting of the $\ell_{1}$ norm has been proposed in several papers and has been shown to have improved performance than a fixed set of weights \cite{CandesReweightedL1}.}
\end{remark}

\subsection{KECM approach for the Spike and Slab Jump Prior}
Now we present a KECM for the spike and slab jump prior.   As with the Laplace prior we treat $X$ as a latent variable.   Let us denote the unknown parameters as $\Phi$ where
\begin{eqnarray}
% \nonumber to remove numbering (before each equation)
\Phi_{1} &=& D \nonumber \\
\Phi_{2} &=& \Gamma \nonumber \\
\Phi_{3} &=& \sigma_{o}^{2}\nonumber \\
\Phi_{4} &=& Z(2:T),\tilde{J}(2:T) \nonumber \\
\Phi_{5} &=& \zeta \nonumber \\
\Phi_{6} &=& \left\{\sigma_{j,i}^{2}(t)\right\}_{i=1,\dots,N,t=1,\dots,T}.  \nonumber
\end{eqnarray}
Here we allow for distinct $\sigma_{j}^{2}$ values for each time and asset.

The E-step as well as the conditional M-steps for $\Phi_{1},\Phi_{2},\Phi_{3}$ are identical to the KECM algorithm for Laplace priors.   The differences for this section are in the conditional M-steps for $J$, $\zeta$ and $\sigma_{j}^{2}$.

First we address the conditional M-step for $J^{(k+1)}$.  Here we need to solve
\begin{eqnarray}\label{eqJumpProbSpike}
[J^{(k+1)}(t),Z^{(k+1)}(t),\tilde{J}^{(k+1)}(t)] &=&\arg\min_{j,z,\tilde{j}} \frac{1}{2}j^{T}( \Gamma^{(k+1)})^{-1} j\nonumber \\
&& \;\;\;\;\;  - j^{T}(\Gamma^{(k+1)})^{-1}\Delta^{(k+1)} - \sum_{i=1}^{N}\log(f(\tilde{j}_{i},z_{i})) \nonumber \\
&& \textnormal{ s.t.  }j_{i} =\tilde{j}_{i}z_{i}
\end{eqnarray}
where
\begin{equation}\label{eq:SpikeSlabPenalty}
  \log f(\tilde{j}_{i},z_{i}) =  \log\left(\zeta 1_{z_{i}=0} +(1-\zeta) 1_{z_{i} = 1}\right)+ \log\left(\frac{1}{\sqrt{2\pi\sigma_{j,i}^{2}}}\exp\left(-\frac{\tilde{j}_{i}^{2}}{2 \sigma_{j,i}^{2}}\right)\right).
\end{equation}
Here we dropped the notation for time dependence.  When restricted to $j_{i} =\tilde{j}_{i}z_{i}$, $-\log(\tilde{j}_{i},z_{i})$ induces a penalty on $j_{i}$.   The penalty is a weighted sum of an $\ell_{0}$ and squared $\ell^{2}$ norm.   A plot of this penalty is shown in Figure \ref{fig:SpikeSlabPen}.
\begin{figure}[h]
    \centering
    \includegraphics[width=5in]{SpikeSlabPen.eps}
    \caption{Spike and slab penalty function for various parameter values.   Here we see that the penalty is a weighted sum of $\ell_{0}$ and squared $\ell_{2}$ norms.}
    \label{fig:SpikeSlabPen}
\end{figure}

The term $-\log(\tilde{j}_{i},z_{i})$ is non-convex and complicates the conditional M-step \eqref{eqJumpProbSpike}.   Hence we seek an approximate maximization through coordinate descent.  Here we divide the problem into tractable 1-dimensional optimization problems with respect to one asset at a time.  The method and equations for implementing coordinate descent are derived in Appendix \ref{SecMCMCAppendixJump} and described below.   For ease of notation we drop the notation denoting dependence on $k$.

Let us define the following conditional mean and variance
\begin{equation}\label{eq:aSpike}
  a(i)=\Delta_{i}(t)+\Gamma_{i,-i}\Gamma_{-i,-i}^{-1}(j_{-i}(t)-\Delta_{-i}(t))
\end{equation}
and
\begin{equation}\label{eq:bSpike}
  b^{2}(i)=\Gamma_{i,i}-\Gamma_{i,-i}\Gamma_{-i,-i}^{-1}\Gamma_{-i,i}
\end{equation}
where the subscript $-i$ is to be interpreted as all indices except $i$.
Then the following rule determines the MAP optimal value of $z_{i}(t)$ conditioned on $j_{-i}(t)$
\begin{eqnarray}\label{eq:SpikeZupdate}
  z_{i|-i}(t) = \begin{cases} 0 \mbox { if } \frac{\zeta}{1-\zeta} \mathcal{N}(0,a(i),b^{2}(i)) > \mathcal{N}(0,a(i),b^{2}(i)+\sigma_{j,i}^{2}(t))  \\
  1 \mbox{ else }\end{cases}
\end{eqnarray}
where $\mathcal{N}(0,a(i),b^{2}(i))$ is the normal PDF with mean $a(i)$ and variance $b^{2}(i)$ evaluated at 0.   An optimal value of $\tilde{J}_{i|-i}(t)$ is then given as
\begin{eqnarray}\label{eq:SlabJupdate}
  \tilde{J}_{i|-i}(t)=\begin{cases} \frac{a}{1+b^{2}\sigma_{j,i}^{-2}(t)} \mbox { if } z_{i|-i}(t) \ne 0 \\
  0  \mbox{ else }
  \end{cases}.
\end{eqnarray}

The mapping defined by equations \eqref{eq:SpikeZupdate} and \eqref{eq:SlabJupdate} is a combination of a thresholding step followed by a shrinkage operation
\begin{eqnarray}\label{eq:SpikeUpdate}
  J_{i|-i}(t)&=&SpikeSlabShrink(a,b^{2}) \nonumber \\
   &\doteq& \begin{cases} 0 &\mbox { if } \frac{\zeta \mathcal{N}(0,a(i),b^{2}(i))}{(1-\zeta)\mathcal{N}(0,a(i),b^{2}(i)+\sigma_{j,i}^{2}(t))} >  1 \\
  \frac{a(i)}{1+b^{2}(i)\sigma_{j,i}^{-2}(t)} & \mbox{ else }
  \end{cases}.
\end{eqnarray}
This spike and slab shrinkage is illustrated in Figure \ref{fig:SpikeSlabShrink}.   As the plots indicate the shrinkage is discontinuous and large values are shrunk more than smaller values.
\begin{figure}[h]
    \centering
    \includegraphics[width=5in]{SpikeSlabShrink.eps}
    \caption{Spike and slab shrinkage function for various parameter values}
    \label{fig:SpikeSlabShrink}
\end{figure}

Equation \eqref{eq:SpikeUpdate} is cycled through all $i=1 \dots N$.  Multiple cycles may also be performed to obtain an improved estimate of $J$.  A summary of the algorithm for the conditional M-step for $J$ is given below in Algorithm \ref{Alg:spikeJ}.
\begin{algorithm}[H]
\caption{Coordinate Descent for Determination of $Z^{(k+1)}(t)$,$\tilde{J}^{(k+1)}(t)$, and $J^{(k+1)}(t)$}
\label{Alg:spikeJ}
\begin{algorithmic}
\STATE  \textbf{Initialize: }Set $J^{(k+1)}(t)=J^{(k)}(t)$, $it$=0, $L>0$
\WHILE{ $it \le L$}
    \STATE $it=it+1$
    \STATE $i=0$
    \WHILE{$i < N$}
        \STATE $i=i+1$
        \STATE Compute $Z_{i}^{(k+1)}(t)$ using equations \eqref{eq:aSpike}, \eqref{eq:bSpike}, and \eqref{eq:SpikeZupdate}
        \STATE Compute $\tilde{J}_{i}^{(k+1)}(t)$ using equations \eqref{eq:aSpike}, \eqref{eq:bSpike}, and \eqref{eq:SlabJupdate}
        \STATE Set $J^{(k+1)}_{i}(t) = Z_{i}^{(k+1)}(t)\tilde{J}_{i}^{(k+1)}(t)$
    \ENDWHILE
\ENDWHILE
\STATE return $J^{(k+1)}(t)$
\end{algorithmic}
\end{algorithm}
Although this method is not guaranteed to solve \eqref{eqJumpProbSpike} it will not increase the value of the objective function compared with $J^{k}(t)$.

Once $J^{(k+1)}$ is obtained, values for $\zeta^{(k+1)}$ and $\sigma_{j}^{2,(k+1)}$ are easily computed through conjugate prior relationships.  First let $P$ be number of zero values in $J(2:T)^{(k+1)}$ and $\tilde{P}=N(T-1)-P$.  Then by conjugate prior relationships the conditional M-steps for $\zeta$ and $\sigma_{j}^{2}$ are
\begin{equation}\label{eq:UpdateZeta}
  \zeta^{(k+1)} = \frac{\alpha_{\zeta}+P}{N(T-1)+\beta_{\zeta}+\alpha_{\zeta}}
\end{equation}
and
\begin{equation}\label{eq:UpdateSigJ}
  \sigma_{j,i}^{2,(k+1)}(t) = \frac{\beta_{j}+0.5(J_{i}(t))^{2}}{\alpha_{j}+1+0.5(Z_{i}(t))}.
\end{equation}

The KECM algorithm for spike and slab models is summarized in Algorithm \ref{Alg:ECMspike}.
\begin{algorithm}[H]
\caption{KECM Algorithm for estimation of $\Gamma$ under Spike and Slab Prior}
\label{Alg:ECMspike}
\begin{algorithmic}
\STATE  \textbf{Initialize: }$\Phi^{(0)},k=0$
\WHILE{ not converged}
\STATE Compute $\bar{X}(t|T), P(t|T),P(t,t-1|T)$ using Kalman smoothing equations for $\Theta^{(k)}$  using equations \eqref{eq:ForwardEq}-\eqref{eq:BackwardRecursion}
\STATE Compute $D^{(k+1)},\Gamma^{(k+1)}$, and $\sigma_{o}^{2,(k+1)}$ using equations \eqref{driftEM}, \eqref{GammaEM}, and \eqref{obsEM} respectively
\STATE For all $t$, compute $\tilde{J}^{(k+1)}(t)$, $Z^{(k+1)}(t)$ using Algorithm \ref{Alg:spikeJ}
\STATE Set $J^{(k+1)}_{i}(t) = Z_{i}^{(k+1)}(t)\tilde{J}_{i}^{(k+1)}(t)$
\STATE Compute $\zeta^{(k+1)}$ using equation \eqref{eq:UpdateZeta}
\STATE Compute $\sigma_{j,i}^{2,(k+1)}(t)$ using equation \eqref{eq:UpdateSigJ} for all $i,t$
\STATE $k=k+1$
\ENDWHILE
\end{algorithmic}
\end{algorithm}

Note that although $J(t)$ is only approximately maximized in each conditional M-step this is still an ECM algorithm.    To see this we can simply redefine $\Phi$ as
\begin{equation*}
  \left[D,\Gamma,\sigma_{o}^{2},J_{1}(2),\dots,J_{N}(2),\dots,J_{1}(T),\dots,J_{N}(T),\zeta,\sigma_{j}^{2}\right].
\end{equation*}
Then the above algorithm is an ECM algorithm for the redefined parameter vector.   The convergence of Algorithm \ref{Alg:ECMspike} is similiar to the proof of the convergence of Algorithm \ref{Alg:ECM} in Appendix \ref{Sec:ConvergeECM}.

\begin{remark}
\textnormal{ A comparison of the spike and slab shrinkage function with the shrinkage function of the $b^{2}-equivalent$ Laplace prior is shown in Figure \ref{fig:SpikeSlabShrinkCompare}.   The Laplace shrinkage function (with parameter $\lambda$)  is defined as
\begin{eqnarray*}
  LaplaceShrink(a,b^{2}) &\doteq& \begin{cases} a-\lambda b^{2} &\mbox { if } a>\lambda b^{2}  \\
  a+\lambda b^{2} & \mbox{ if } a<-\lambda b^{2} \\
  0 &\mbox{ else }
  \end{cases}.
\end{eqnarray*}
The graphs illustrate advantages and disadvantages of the Laplace prior.   One notable disadvantage is that for large $\sigma_{j}^{2}$ the Laplace prior has a large bias relative to spike and slab priors.   However for small $\sigma_{j}^{2}$ and large values of $a$ we see that the Laplace prior is less biased than the spike and slab.   This can be attributed to the quadratic penalty induced by the spike and slab prior which penalizes large jumps more heavily than the Laplace prior.}
\end{remark}
\begin{figure}[h]
    \centering
    \includegraphics[width=5in]{LaplaceSpikeCompare.eps}
    \caption{Shrinkage Functions of the spike and slab and the corresponding $b^{2}-equivalent$ Laplace prior}
    \label{fig:SpikeSlabShrinkCompare}
\end{figure}

%To facilitate derivation of the conditional M-step recall from equation \ref{eq:DefJump} $J=Z\tilde{J}$.   Thus we factor $J^{(k+1)}$ into two terms %$J^{(k+1)}(t)=Z^{(k+1)}(t)\tilde{J^{(k+1)}}(t)$.   With this factorization we have the following optimization problem




==> Simulation.tex <==
\section{Simulation Results}

==> SpikeSlabConv.tex <==
\subsection{Results for Spike and Slab Penalty}
Suppose that the there are $M$ jumps at time $t$ and without loss of generality we shall assume that the first $M$ asset prices have jumps.   Since $t$ is fixed we shall drop the notation for $t$.  For notation let us partition the covariance matrix $\Gamma$ as
\begin{equation*}
  \Gamma = \left(
     \begin{array}{cc}
       \Gamma_{11} & \Gamma_{12} \\
       \Gamma_{21} & \Gamma_{22} \\
     \end{array}
   \right)
\end{equation*}
where $\Gamma_{11}$ is the $M \times M$ submatrix corresponding to assets $1$ to $M$, and $\Gamma_{22}$ is the $N-M \times N-M$ submatrix corresponding to assets $M+1$ to $N$.   Let us denote $\Gamma_{max}$,$\Gamma_{min}$,$\sigma_{j,max}^{2}$,$\sigma_{j,min}^{2}$ as the maximum and minimum of the diagonal elements of $\Gamma$ and $\sigma_{j}^{2}$
Also define the diagonal matrix
\begin{equation*}
  D_{J} =diag(\sigma_{j,1}^{2}, \dots, \sigma_{j,M}^{2})   GENERALIZE
\end{equation*}
and the matrix
\begin{equation*}
H =\Gamma_{11} + D_{J}.
\end{equation*}

Throughout this section we assume the following
\begin{itemize}
  \item A1) $||\Gamma_{12}\Gamma_{22}^{-1}||_{\infty} < c_{1}$,$||\Gamma_{i,-i}\Gamma_{-i,-i}^{-1}||_{\infty} < c_{1}$  for some $0 \le c_{1} <1$
  \item A2) The minimum eigenvalue of $\Gamma$, $\sigma_{min}$, is greater than $c_{2}$ where $c_{2}>0$
  \item A3) $||\hat{X}-X||_{\infty}<\frac{\epsilon_{1}}{2}<1$
  \item A4) $\hat{\Gamma}=\Gamma$
  \item A5) $|| Q'\left(\Gamma +Q\right)^{-1}  - [I, -\Gamma_{12}\Gamma_{22}^{-1}]||_{\infty} < \epsilon_{2}$
  where
  \begin{equation*}
    Q=diag(\sigma_{j,1}^{2}, \dots, \sigma_{j,M}^{2},0,\dots,0)
  \end{equation*}
  \begin{equation*}
    Q'=[ D_{J} , 0_{M \times (N-M)}]
  \end{equation*}
and where $0_{M \times N-M}$ is a $M \times (N-M)$ matrix of zeros.   GENERALIZE FOR ALL SIZE DIAGONAL
\end{itemize}
Assumption 1 is a mutual incoherence property which is a common condition needed for establishing support recovery.   Assumption 3 simply states that the posterior mean of $X$ is close to the true value.    Assumption 4 states that the estimated covariance matrix equals the true covariance.   An extension of this analysis could consider the case $||\hat{\Gamma}-\Gamma||_{\infty} < \epsilon$.   The following lemma shows that assumption 5 is not overly restrictive if $\sigma_{j,i}^2$ is large.
\begin{lemma}
Let $Q,Q'$ be defined as in assumption A5.  Let $q=\inf\left\{\sigma_{j,i}^{2}: i \in 1, \dots M\right\}$.   Then
\begin{equation*}
  \lim_{q \rightarrow \infty} ||Q'\left(\Gamma +Q\right)^{-1} - [I, -\Gamma_{12}\Gamma_{22}^{-1}]||_{\infty}=0
\end{equation*} GENERALIZE FOR ALL SIZE DIAGONAL
\end{lemma}
\begin{proof}
By the matrix inversion results for partitioned matrices we have
\begin{equation*}
Q'\left(\Gamma +Q\right)^{-1} = D_{J}[ (H - \Gamma_{12}\Gamma_{22}^{-1}\Gamma_{21})^{-1},-H^{-1}\Gamma_{12}(\Gamma_{22}-\Gamma_{21}^{-1}H^{-1}\Gamma_{12})^{-1}]
\end{equation*}
Thus we have
\begin{equation*}
  \lim_{q \rightarrow \infty} ||Q'\left(\Gamma +Q\right)^{-1} - [I, -\Gamma_{12}\Gamma_{22}^{-1}]||_{\infty}=0.
\end{equation*}
\end{proof}

\begin{lemma}\label{LemmaAequiv}
Let $\hat{J}_{i}=( Q'(Q+\Gamma)^{-1}\Delta)_{i}$ for $i \in \{1,\dots,M\}$ and $0$ else.    Let $i \in \{1,\dots,M\}$.  Then $\hat{J}_{i} = \frac{a(i)}{1+b^{2}(i)\sigma_{j,i}^{-2}}$ where $a(i),b(i)$ are defined in equations XXX and XXX using $j=J$.
\end{lemma}

\begin{proof}
Note that
\begin{equation*}
 \hat{J} =\E[J|\Delta,Z_{M+1:N}=0,Z_{1:M}=1]
\end{equation*}
and
\begin{equation*}
    \frac{a(i)}{1+b^{2}(i)\sigma_{j,i}^{-2}} =\E[J_{i}|\Delta,Z_{M+1:N}=0,Z_{1:M}=1,J_{-i}=\hat{J}_{-i}].
\end{equation*}
Here the expectation is conditioned on the parameters $\Gamma, \sigma_{o}^{2},D,\sigma_{j}^{2}$.   Since the conditional posterior distribution is normal it follows that
\begin{equation*}
\E[J_{i}|\Delta,Z_{M+1:N}=0,Z_{1:M}=1,J_{-i}=\hat{J}_{-i}]=\hat{J}_{i}.
\end{equation*}
Thus $\hat{J}_{i} = \frac{a}{1+b^{2}\sigma_{j,i}^{-2}}$.
\end{proof}

Let

 \begin{equation}\label{SSsigQQ}
   \sigma_{q}^{2} =4(N^{2}\epsilon_{2}^{2} \Gamma_{max}) \vee 4\Gamma_{max}.
 \end{equation}
and
 \begin{equation}\label{SSeta}
   \eta(j) =\epsilon_{2}||j||_{1} - (1+N\epsilon_{2}+c_{1}(N-M))\epsilon_{1}.
 \end{equation}
  
\begin{lemma}\label{LemmaSSClose}
Suppose $J=j$, and $j_{i} \ne 0$ for $i \le M$ and $j_{i}=0$ else . Let $\hat{J}_{i}=( Q'(Q+\Gamma)^{-1}\Delta)_{i}$ for $i \in \{1,\dots,M\}$ and $0$ else. Then for $i \le M$
\begin{equation*}
  \textnormal{Pr}(|\hat{J}_{i}-J_{i}|<\delta) \ge \textnormal{erf}\left(\frac{\delta'}{\sqrt{2\sigma_{q}^2}}\right)
\end{equation*}
and
\begin{equation*}
  \textnormal{Pr}(|\hat{J}_{i}-\Delta_{i}|<\delta) \ge \textnormal{erf}\left(\frac{\delta'}{\sqrt{2\sigma_{q}^2}}\right)
\end{equation*}

where
\begin{equation*}
  \delta^{'} =( \delta - \eta(j) ) \vee 0.
\end{equation*}
and

\end{lemma}
\begin{proof}
Let $i \le M$.  From assumption A3, $\Delta -J +v$ is $\mathcal{N}(0,\Gamma)$ for some $v$ such that $||v||_{\infty}<\epsilon_{1}$.  Then
\begin{eqnarray*}
% \nonumber to remove numbering (before each equation)
  \hat{J}_{i}-J_{i} &=& ( Q'(Q+\Gamma)^{-1}\Delta)_{i} - J_{i} \\
  &=& ( Q'(Q+\Gamma)^{-1}J)_{i} - J_{i} + ( Q'(Q+\Gamma)^{-1}q)_{i} + ( Q'(Q+\Gamma)^{-1}v)_{i}
\end{eqnarray*}
where $q$ is $\mathcal{N}(0,\Gamma)$.  By A5 we have
\begin{eqnarray*}
  |( Q'(Q+\Gamma)^{-1}j)_{i} - J_{i}|&<&\epsilon_{2} ||J||_{1} \\
  &=& \epsilon_{2} ||j||_{1}
\end{eqnarray*}
and
\begin{eqnarray*}
  |( Q'(Q+\Gamma)^{-1}v)_{i}|&<&(1+\epsilon_{2})\epsilon_{1} + (M-1)\epsilon_{2}\epsilon_{1} + (c_{1}+\epsilon_{2})\epsilon_{1}(N-M) \\
  &=& (1+N\epsilon_{2}+c_{1}(N-M))\epsilon_{1}
\end{eqnarray*}
Also by A5
\begin{eqnarray*}
  ( Q'(Q+\Gamma)^{-1}q)_{i}=([I,\Gamma_{12}\Gamma_{22}^{-1}]q)_{i} + w^{T}q
\end{eqnarray*}
where $||w||_{\infty}<\epsilon_{2}$.
The first term is normally distributed with zero mean and variance less than $\Gamma_{\max}$.   The second term is normally distributed with zero mean and variance less than
\begin{equation*}
  N^{2}\epsilon_{2}^{2} \Gamma_{max}
\end{equation*}
Thus $( Q'(Q+\Gamma)^{-1}q)_{i}$ is zero mean normally distributed with variance greater than or equal to $\sigma_{q}^{2}$.



Then by the triangle inequality $|\hat{J}_{i}-J_{i}|<\delta$ if
\begin{equation*}
  | ( Q'(Q+\Gamma)^{-1}q)_{i}| < \delta - \epsilon_{2}||j||_{1} - (1+N\epsilon_{2}+c_{1}(N-M))\epsilon_{1}
\end{equation*}


Then
\begin{eqnarray*}
  \textnormal{Pr}(|\hat{J}_{i}-J_{i}|<\delta) &\ge& Pr(| ( Q'(Q+\Gamma)^{-1}q)_{i}| < \delta') \\
  &\ge&  \textnormal{erf}\left(\frac{\delta'}{\sqrt{2\sigma_{q}^2}}\right)
\end{eqnarray*}

The proof that
\begin{equation*}
  \textnormal{Pr}(|\hat{J}_{i}-\Delta_{i}|<\delta) \ge \textnormal{erf}\left(\frac{\delta'}{\sqrt{2\sigma_{q}^2}}\right)
\end{equation*}
is similar.

\end{proof}

\begin{comment}
\begin{lemma}
Suppose $J=j$, and $j_{i} \ne 0$ for $i \le M$ and $j_{i}=0$ else . Let $\hat{J}_{i}=( Q'(Q+\Gamma)^{-1}\Delta)_{i}$ for $i \in \{1,\dots,M\}$ and $0$ else.  Then for $i \le M$
\begin{equation*}
  Pr(|\hat{J}_{i}-\Delta_{i}|<\delta) > ???
\end{equation*}
\end{lemma}
\begin{proof}
Let $1 \le i \le M$.   From assumption A3, $\Delta_{i} -J_{i} +v_{i}$ is $\mathcal{N}(0,\Gamma)$ for some $v$ such that $|v_{i}|<\epsilon_{1}$.   Thus
\begin{eqnarray*}
% \nonumber to remove numbering (before each equation)
  \hat{J}_{i}-\Delta_{i} &=& ( Q'(Q+\Gamma)^{-1}\Delta)_{i} - \Delta_{i} \\
  &=& ( Q'(Q+\Gamma)^{-1}J)_{i} - J_{i} + ( Q'(Q+\Gamma)^{-1}q)_{i}-q_{i} + ( Q'(Q+\Gamma)^{-1}v)_{i} -v_{i}
\end{eqnarray*}
From the proof of the prior lemma
\begin{eqnarray*}
  |( Q'(Q+\Gamma)^{-1}j)_{i} - J_{i}|&<& \epsilon_{2} ||j||_{1}
\end{eqnarray*}
\begin{eqnarray*}
  |( Q'(Q+\Gamma)^{-1}v)_{i}-v_{i}|&<& (1+N\epsilon_{2}+c_{1}(N-M))\epsilon_{1}
\end{eqnarray*}
and
\begin{eqnarray*}
  |( Q'(Q+\Gamma)^{-1}q)_{i}-q_{i}|
\end{eqnarray*}
is zero mean normally distributed with variance greater than or equal to $\sigma_{q}^{2}$.   Thus
\end{proof}
\begin{eqnarray*}
  Pr(|\hat{J}_{i}-\Delta_{i}|<\delta) &\ge& Pr(|( Q'(Q+\Gamma)^{-1}q)_{i}-q_{i}|<\delta') \\
&\ge& \textnormal{erf}\left(\frac{\delta''}{\sqrt{2(\sigma_{q}^{2})}}\right).
\end{eqnarray*}
\end{comment}
%\begin{lemma}
%Let $b(i)$ be defined as in equation XXX.   Then
%\begin{equation*}
%  s \le b(i) \le \Gamma_{max}
%\end{equation*}
%where $s$ is the minimum eigenvalue of $\hat{\Gamma}$.
%\end{lemma}
%\begin{proof}
%Since $\Gamma_{-i,-i}$ is positive semidefinite, $b(i) \le \Gamma_{max}$.   Define $w$ as $w_{i}=1$, $w_{j}=\hat{Gamma}_{i,-i}\Gamma{-i,j}$ for $j \ne i$.   Then \begin{equation*}
%  b(i)= w^{T}\hat{\Gamma}w \ge s||w||_{\ell_{2}} > s.
%\end{equation*}
%\end{proof}

The update equation for $z_{i|-i}$ given in equation XXX, may re-written as
\begin{eqnarray*}
  z_{i|-i} = \begin{cases} 0 \mbox { if } a(i)^{2} < T_{i}\\
  1 \mbox{ else }\end{cases}
\end{eqnarray*}
where
\begin{equation*}
  T_{i} =  \left(\log\left(\frac{\zeta}{1-\zeta}\right)+0.5\log\left(\frac{b^{2}(i)+\sigma_{j,i}^{2}}{b^{2}(i)}\right)\right)\frac{2b^{2}(i)(b^{2}(i)+\sigma_{j,i}^{2})}{\sigma_{j,i}^{2}}  \end{equation*}
The next two lemmas determine the probability that $z_{i|-i}=1$.

\begin{lemma}
Suppose $J_{i} \ne 0$ for $i \le M$ and $J_{i}=0$ else.   Let $\hat{J}_{i}=( Q'(Q+\Gamma)^{-1}\Delta)_{i}$ for $i \le M$ and $\hat{J}_{i}=0$ else.  If $|J_{i}|-\sqrt{T_{i}}>\eta$.  Then for $j=\hat{J}$ and $1 \le i \le M$
\begin{equation*}
  \textnormal{Pr}(z_{i|-i}=1)> \textnormal{erf}\left(\frac{|J_{i}|-\sqrt{T_{i}}-\eta(j)}{\sqrt{2\sigma_{q}^2}}\right)
\end{equation*}
\end{lemma}
\begin{proof}
Let $i \in \{1, \dots M\}$.   Since $z_{i|-i}=1$ if and only  $a(i)^{2} \ge T_{i}$ it follows that 
\begin{equation*}
  \textnormal{Pr}(z_{i|-i}=1)= \textnormal{Pr}(a(i)^{2} \ge T_{i})
\end{equation*}
By equation XXX and lemma \ref{LemmaAequiv} we have $|a_{i}|>|\hat{J}_{i}|$.
Thus 
\begin{eqnarray*}
  \textnormal{Pr}(z_{i|-i}=1) &>& \textnormal{Pr}(\hat{J}_{i}^{2} \ge T_{i}) \\
&>&\textnormal{Pr}(\hat{J}_{i}-J_{i} \le |J_{i}|-T_{i}).
\end{eqnarray*}
By lemma \ref{LemmaSSClose}
\begin{eqnarray*}
  \textnormal{Pr}(z_{i|-i}=1) &>&  \textnormal{erf}\left(\frac{|J_{i}|-\sqrt{T_{i}}-\eta(j)}{\sqrt{2\sigma_{q}^2}}\right).
\end{eqnarray*}
\end{proof} 
\begin{lemma}
Suppose $J_{i} \ne 0$ for $i \le M$ and $J_{i}=0$ else.   If $|J_{i}|-\sqrt{T_{i}}>\eta$.  Then for $1 \le i \le M$
\begin{equation*}
  \textnormal{Pr}(z_{i|-i}=1)> \textnormal{erf}\left(\frac{|J_{i}|-\sqrt{T_{i}}-\eta}{\sqrt{2\sigma_{q}^2}}\right)
\end{equation*}
\end{lemma}
\begin{proof}
Let $i \in \{1, \dots M\}$.   Since $z_{i|-i}=1$ if and only  $a(i)^{2} \ge T_{i}$ it follows that
\begin{equation*}
  \textnormal{Pr}(z_{i|-i}=1)= \textnormal{Pr}(a(i)^{2} \ge T_{i})
\end{equation*}
Let $\hat{J}_{i}=( Q'(Q+\Gamma)^{-1}\Delta)_{i}$.    By equation XXX and lemma \ref{LemmaAequiv} we have $|a_{i}|>|\hat{J}_{i}|$.
Thus
\begin{eqnarray*}
  \textnormal{Pr}(z_{i|-i}=1) &>& \textnormal{Pr}(\hat{J}_{i}^{2} \ge T_{i}) \\
&>&\textnormal{Pr}(\hat{J}_{i}-J_{i} \le |J_{i}|-T_{i}).
\end{eqnarray*}
By lemma \ref{LemmaSSClose}
\begin{eqnarray*}
  \textnormal{Pr}(z_{i|-i}=1) &>&  \textnormal{erf}\left(\frac{|J_{i}|-\sqrt{T_{i}}-\eta}{\sqrt{2\sigma_{q}^2}}\right).
\end{eqnarray*}
\end{proof}
%%%%%%%%%%%%%%%%%%
\begin{lemma}
Suppose $J_{i} \ne 0$ for $i \le M$ and $J_{i}=0$ else.   Let $\hat{J}_{i}=( Q'(Q+\Gamma)^{-1}\Delta)_{i}$ for $i \le M$ and $\hat{J}_{i}=0$ else.  Then for $j=\hat{J}$ and $i>M$
\begin{equation*}
  \textnormal{Pr}(z_{i|-i}=0)> %%%\textnormal{erf}\left(\frac{|J_{i}|-\sqrt{T_{i}}-\eta}{\sqrt{2\sigma_{q}^2}}\right)
\end{equation*}
\end{lemma}
\begin{proof}
Let $i>M$.  Note that 
\begin{equation*}
  \textnormal{Pr}(z_{i|-i}=0)= \textnormal{Pr}(a(i)^{2} < T_{i}).
\end{equation*} 
By assumption 1
\begin{equation*}
|a(i)| < |\Delta_{i} + \Gamma_{i,-i}\Gamma_{-i,-i}(\Delta)| + |c_{1}\sum_{k=1}^{M}(j_{k}-\Delta_{k})|. 
\end{equation*}

\end{proof}



==> SpikeSlabConv2.tex <==
\subsection{Results for Spike and Slab Penalty}
In this section we show that the oracle solution is a fixed point of Algorithm ?? with high probability.   The oracle solution is the MAP estimate of the jumps assuming the support of the jumps is known.  We shall define the oracle solution as $\hat{J}$.

Suppose that the there are $M$ jumps at time $t$ and without loss of generality we assume they occur in first $M$ assets.   Since $t$ is fixed we shall drop the notation for $t$.  For notation let us partition the covariance matrix $\Gamma$ as
\begin{equation*}
  \Gamma = \left(
     \begin{array}{cc}
       \Gamma_{11} & \Gamma_{12} \\
       \Gamma_{21} & \Gamma_{22} \\
     \end{array}
   \right)
\end{equation*}
where $\Gamma_{11}$ is the $M \times M$ submatrix corresponding to assets $1$ to $M$, and $\Gamma_{22}$ is the $N-M \times N-M$ submatrix corresponding to assets $M+1$ to $N$.   Let us denote $\Gamma_{max}$,$b_{max}$ as the maximum elements of $\Gamma$ and $b$ (equation X) respectively. 
Also for later use define the diagonal matrix
\begin{equation*}
  D_{J} =diag(\sigma_{j,1}^{2}, \dots, \sigma_{j,M}^{2})   
\end{equation*}
and the matrix
\begin{equation*}
H =\Gamma_{11} + D_{J}.
\end{equation*}

Throughout this section we assume the following
\begin{itemize}
  \item A1) $|( \Gamma_{i,-i}\Gamma_{-i,-i}^{-1})_{k}| < c_{1}$  for some $c_{1}>0$ and all $k \le M$
  \item A2) $\hat{X}=X$
  \item A3) $\hat{\Gamma}=\Gamma$
  \item A4) $|| Q'\left(\Gamma +Q\right)^{-1}  - [I, -\Gamma_{12}\Gamma_{22}^{-1}]||_{\infty} < \epsilon_{1}$
  where
  \begin{equation*}
    Q=diag(\sigma_{j,1}^{2}, \dots, \sigma_{j,M}^{2},0,\dots,0)
  \end{equation*}
  \begin{equation*}
    Q'=[ D_{J} , 0_{M \times (N-M)}]
  \end{equation*}
and where $0_{M \times N-M}$ is a $M \times (N-M)$ matrix of zeros.  
\end{itemize}
Assumption 1 is a mutual incoherence property which is a common condition needed for establishing support recovery.   Assumption 2 simply states that the estimate of $X$ is exact.    Assumption 3 states that the estimated covariance matrix equals the true covariance.  The following lemma shows that assumption 4 is not overly restrictive if $\sigma_{j,i}^2$ is large.
\begin{lemma}
Let $Q,Q'$ be defined as in assumption 4.  Let 
\begin{equation*}
  q=\inf\left\{\sigma_{j,i}^{2}: i \in 1, \dots M\right\}.
\end{equation*}
 Then
\begin{equation*}
  \lim_{q \rightarrow \infty} ||Q'\left(\Gamma +Q\right)^{-1} - [I, -\Gamma_{12}\Gamma_{22}^{-1}]||_{\infty}=0.
\end{equation*} 
\end{lemma}
\begin{proof}
By the matrix inversion results for partitioned matrices we have
\begin{equation*}
Q'\left(\Gamma +Q\right)^{-1} = D_{J}[ (H - \Gamma_{12}\Gamma_{22}^{-1}\Gamma_{21})^{-1},-H^{-1}\Gamma_{12}(\Gamma_{22}-\Gamma_{21}^{-1}H^{-1}\Gamma_{12})^{-1}]
\end{equation*}
As $q$ goes to infinity $H^{-1}$ goes to zero and $D_{J}H^{-1}$ goes to $I$.   Thus
\begin{equation*}
  \lim_{q \rightarrow \infty} ||Q'\left(\Gamma +Q\right)^{-1} - [I, -\Gamma_{12}\Gamma_{22}^{-1}]||_{\infty}=0.
\end{equation*}
\end{proof}

The next lemma follows from the equation for the conditional mean of normal random variable.
\begin{lemma}
The oracle solution to the jump estimation problem is given as $\hat{J}$ where $\hat{J}_{i}=( Q'(Q+\Gamma)^{-1}\Delta)_{i}$ for $i \in \{1,\dots,M\}$ and $0$ else.
\end{lemma}

The next lemma establishes an important relationship regarding the oracle solution.
\begin{lemma}\label{LemmaAequiv}
Let $\hat{J}$ be the oracle solution.   Let $i \in \{1,\dots,M\}$.  Then $\hat{J}_{i} = \frac{a(i)}{1+b^{2}(i)\sigma_{j,i}^{-2}}$ where $a(i),b(i)$ are defined in equations XXX and XXX using $j=J$.
\end{lemma}

\begin{proof}
Note that
\begin{equation*}
 \hat{J} =\E[J|\Delta,Z_{M+1:N}=0,Z_{1:M}=1]
\end{equation*}
and
\begin{equation*}
    \frac{a(i)}{1+b^{2}(i)\sigma_{j,i}^{-2}} =\E[J_{i}|\Delta,Z_{M+1:N}=0,Z_{1:M}=1,J_{-i}=\hat{J}_{-i}].
\end{equation*}
Here the expectation is conditioned on the parameters $\Gamma, \sigma_{o}^{2},D,\sigma_{j}^{2}$.   Since the conditional posterior distribution is normal it follows that
\begin{equation*}
\E[J_{i}|\Delta,Z_{M+1:N}=0,Z_{1:M}=1,J_{-i}=\hat{J}_{-i}]=\hat{J}_{i}.
\end{equation*}
Thus $\hat{J}_{i} = \frac{a}{1+b^{2}\sigma_{j,i}^{-2}}$.
\end{proof}

Our next result shows that the oracle solution is close to the true solution under our assumptions.   First we introduce some notation.
 \begin{equation}\label{SSsigQQ}
   \sigma_{q}^{2} =( N\epsilon_{1}\sqrt{\Gamma_{max}} +\sqrt{b_{max}})^{2}.
 \end{equation}
and
 \begin{equation}\label{SSeta}
   \eta(j) =\epsilon_{1}||j||_{1}
 \end{equation}

\begin{lemma}\label{LemmaSSClose}
Suppose $J=j$, and $j_{i} \ne 0$ for $i \le M$ and $j_{i}=0$ else . Let Let $\hat{J}$ be the oracle solution.  Then for $i \le M$
\begin{equation*}
  \textnormal{Pr}(|\hat{J}_{i}-J_{i}|<\delta) \ge \textnormal{erf}\left(\frac{\delta'}{\sqrt{2\sigma_{q}^2}}\right)
\end{equation*}
and
\begin{equation*}
  \textnormal{Pr}(|\hat{J}_{i}-\Delta_{i}|<\delta) \ge \textnormal{erf}\left(\frac{\delta'}{\sqrt{2\sigma_{q}^2}}\right)
\end{equation*}
where
\begin{equation*}
  \delta^{'} =( \delta - \eta(j) ) \vee 0.
\end{equation*}
\end{lemma}
\begin{proof}
Let $i \le M$.  From assumption A2, $\Delta -J$ is $\mathcal{N}(0,\Gamma)$.  Then
\begin{eqnarray*}
% \nonumber to remove numbering (before each equation)
  \hat{J}_{i}-J_{i} &=& ( Q'(Q+\Gamma)^{-1}\Delta)_{i} - J_{i} \\
  &=& ( Q'(Q+\Gamma)^{-1}J)_{i} - J_{i} + ( Q'(Q+\Gamma)^{-1}q)_{i}
\end{eqnarray*}
where $q$ is $\mathcal{N}(0,\Gamma)$.  By A4 we have
\begin{eqnarray*}
  |( Q'(Q+\Gamma)^{-1}j)_{i} - J_{i}|&<&\epsilon_{1} ||J||_{1} \\
  &=& \epsilon_{1} ||j||_{1}
\end{eqnarray*}
Also by A4
\begin{eqnarray*}
  ( Q'(Q+\Gamma)^{-1}q)_{i}=([I,-\Gamma_{12}\Gamma_{22}^{-1}]q)_{i} + w^{T}q
\end{eqnarray*}
where $||w||_{\infty}<\epsilon_{1}$.
The first term is normally distributed with zero mean and variance less than $b_{max}$.   The second term is normally distributed with zero mean and variance less than
\begin{equation*}
  N^{2}\epsilon_{1}^{2} \Gamma_{max}.
\end{equation*}
Thus $( Q'(Q+\Gamma)^{-1}q)_{i}$ is zero mean normally distributed with variance less than or equal to $\sigma_{q}^{2}$.

By the triangle inequality $|\hat{J}_{i}-J_{i}|<\delta$ if
\begin{equation*}
  | ( Q'(Q+\Gamma)^{-1}q)_{i}| < \delta - \epsilon_{1}||j||_{1}
\end{equation*}
Thus
\begin{eqnarray*}
  \textnormal{Pr}(|\hat{J}_{i}-J_{i}|<\delta) &\ge& Pr(| ( Q'(Q+\Gamma)^{-1}q)_{i}| < \delta') \\
  &\ge&  \textnormal{erf}\left(\frac{\delta'}{\sqrt{2\sigma_{q}^2}}\right)
\end{eqnarray*}

The proof that
\begin{equation*}
  \textnormal{Pr}(|\hat{J}_{i}-\Delta_{i}|<\delta) \ge \textnormal{erf}\left(\frac{\delta'}{\sqrt{2\sigma_{q}^2}}\right)
\end{equation*}
is similar.

\end{proof}

\begin{comment}
\begin{lemma}
Suppose $J=j$, and $j_{i} \ne 0$ for $i \le M$ and $j_{i}=0$ else . Let $\hat{J}_{i}=( Q'(Q+\Gamma)^{-1}\Delta)_{i}$ for $i \in \{1,\dots,M\}$ and $0$ else.  Then for $i \le M$
\begin{equation*}
  Pr(|\hat{J}_{i}-\Delta_{i}|<\delta) > ???
\end{equation*}
\end{lemma}
\begin{proof}
Let $1 \le i \le M$.   From assumption A3, $\Delta_{i} -J_{i} +v_{i}$ is $\mathcal{N}(0,\Gamma)$ for some $v$ such that $|v_{i}|<\epsilon_{1}$.   Thus
\begin{eqnarray*}
% \nonumber to remove numbering (before each equation)
  \hat{J}_{i}-\Delta_{i} &=& ( Q'(Q+\Gamma)^{-1}\Delta)_{i} - \Delta_{i} \\
  &=& ( Q'(Q+\Gamma)^{-1}J)_{i} - J_{i} + ( Q'(Q+\Gamma)^{-1}q)_{i}-q_{i} + ( Q'(Q+\Gamma)^{-1}v)_{i} -v_{i}
\end{eqnarray*}
From the proof of the prior lemma
\begin{eqnarray*}
  |( Q'(Q+\Gamma)^{-1}j)_{i} - J_{i}|&<& \epsilon_{2} ||j||_{1}
\end{eqnarray*}
\begin{eqnarray*}
  |( Q'(Q+\Gamma)^{-1}v)_{i}-v_{i}|&<& (1+N\epsilon_{2}+c_{1}(N-M))\epsilon_{1}
\end{eqnarray*}
and
\begin{eqnarray*}
  |( Q'(Q+\Gamma)^{-1}q)_{i}-q_{i}|
\end{eqnarray*}
is zero mean normally distributed with variance greater than or equal to $\sigma_{q}^{2}$.   Thus
\end{proof}
\begin{eqnarray*}
  Pr(|\hat{J}_{i}-\Delta_{i}|<\delta) &\ge& Pr(|( Q'(Q+\Gamma)^{-1}q)_{i}-q_{i}|<\delta') \\
&\ge& \textnormal{erf}\left(\frac{\delta''}{\sqrt{2(\sigma_{q}^{2})}}\right).
\end{eqnarray*}
\end{comment}
%\begin{lemma}
%Let $b(i)$ be defined as in equation XXX.   Then
%\begin{equation*}
%  s \le b(i) \le \Gamma_{max}
%\end{equation*}
%where $s$ is the minimum eigenvalue of $\hat{\Gamma}$.
%\end{lemma}
%\begin{proof}
%Since $\Gamma_{-i,-i}$ is positive semidefinite, $b(i) \le \Gamma_{max}$.   Define $w$ as $w_{i}=1$, $w_{j}=\hat{Gamma}_{i,-i}\Gamma{-i,j}$ for $j \ne i$.   Then \begin{equation*}
%  b(i)= w^{T}\hat{\Gamma}w \ge s||w||_{\ell_{2}} > s.
%\end{equation*}
%\end{proof}

The update equation for $z_{i|-i}$ given in equation XXX, may re-written as
\begin{eqnarray*}
  z_{i|-i} = \begin{cases} 0 \mbox { if } a(i)^{2} < T_{i}\\
  1 \mbox{ else }\end{cases}
\end{eqnarray*}
where
\begin{equation*}
  T_{i} =  \left(\log\left(\frac{\zeta}{1-\zeta}\right)+0.5\log\left(\frac{b^{2}(i)+\sigma_{j,i}^{2}}{b^{2}(i)}\right)\right)\frac{2b^{2}(i)(b^{2}(i)+\sigma_{j,i}^{2})}{\sigma_{j,i}^{2}}  \end{equation*}
Denote $T_{max}$ and $T_{min}$ as the max and min of $T$.

\begin{lemma}
Suppose $J_{i} \ne 0$ for $i \le M$ and $J_{i}=0$ else.   Let $\hat{J}$ be the oracle solution.  If $|J_{i}|-\sqrt{T_{i}}>\eta$.  Then for $j=\hat{J}$ and $1 \le i \le M$
\begin{equation*}
  \textnormal{Pr}(z_{i|-i}=1)> \textnormal{erf}\left(\frac{|J_{i}|-\sqrt{T_{i}}-\eta(j)}{\sqrt{2\sigma_{q}^2}}\right)
\end{equation*}
\end{lemma}
\begin{proof}
Let $i \in \{1, \dots M\}$.   Since $z_{i|-i}=1$ if and only  $a(i)^{2} \ge T_{i}$ it follows that
\begin{equation*}
  \textnormal{Pr}(z_{i|-i}=1)= \textnormal{Pr}(a(i)^{2} \ge T_{i})
\end{equation*}
By equation XXX and lemma \ref{LemmaAequiv} we have $|a_{i}|>|\hat{J}_{i}|$.
Thus
\begin{eqnarray*}
  \textnormal{Pr}(z_{i|-i}=1) &>& \textnormal{Pr}(\hat{J}_{i}^{2} \ge T_{i}) \\
&>&\textnormal{Pr}(\hat{J}_{i}-J_{i} \le |J_{i}|-T_{i}).
\end{eqnarray*}
By lemma \ref{LemmaSSClose}
\begin{eqnarray*}
  \textnormal{Pr}(z_{i|-i}=1) &>&  \textnormal{erf}\left(\frac{|J_{i}|-\sqrt{T_{i}}-\eta(j)}{\sqrt{2\sigma_{q}^2}}\right).
\end{eqnarray*}
\end{proof}
\begin{lemma}
Suppose $J_{i} \ne 0$ for $i \le M$ and $J_{i}=0$ else.   If $|J_{i}|-\sqrt{T_{i}}>\eta$.  Then for $1 \le i \le M$
\begin{equation*}
  \textnormal{Pr}(z_{i|-i}=1)> \textnormal{erf}\left(\frac{|J_{i}|-\sqrt{T_{i}}-\eta(J)}{\sqrt{2\sigma_{q}^2}}\right)
\end{equation*}
\end{lemma}
\begin{proof}
Let $i \in \{1, \dots M\}$.   Since $z_{i|-i}=1$ if and only  $a(i)^{2} \ge T_{i}$ it follows that
\begin{equation*}
  \textnormal{Pr}(z_{i|-i}=1)= \textnormal{Pr}(a(i)^{2} \ge T_{i})
\end{equation*}
Let $\hat{J}_{i}=( Q'(Q+\Gamma)^{-1}\Delta)_{i}$.    By equation XXX and lemma \ref{LemmaAequiv} we have $|a_{i}|>|\hat{J}_{i}|$.
Thus
\begin{eqnarray*}
  \textnormal{Pr}(z_{i|-i}=1) &>& \textnormal{Pr}(|\hat{J}_{i}| \ge \sqrt{T_{i}}) \\
&>&\textnormal{Pr}(|\hat{J}_{i}-J_{i}| \le |J_{i}|-T_{i}).
\end{eqnarray*}
By lemma \ref{LemmaSSClose}
\begin{eqnarray*}
  \textnormal{Pr}(z_{i|-i}=1) &>&  \textnormal{erf}\left(\frac{|J_{i}|-\sqrt{T_{i}}-\eta}{\sqrt{2\sigma_{q}^2}}\right).
\end{eqnarray*}
\end{proof}
%%%%%%%%%%%%%%%%%%
\begin{lemma}
Suppose $J_{i} \ne 0$ for $i \le M$ and $J_{i}=0$ else.   Let $\hat{J}_{i}=( Q'(Q+\Gamma)^{-1}\Delta)_{i}$ for $i \le M$ and $\hat{J}_{i}=0$ else.  Then for $j=\hat{J}$
\begin{equation*}
  \textnormal{Pr}(z_{i|-i}=0, \forall i>M)> %%%\textnormal{erf}\left(\frac{|J_{i}|-\sqrt{T_{i}}-\eta}{\sqrt{2\sigma_{q}^2}}\right)
\end{equation*}
\end{lemma}
\begin{proof}
Let $i>M$.  Note that
\begin{equation*}
  \textnormal{Pr}(z_{i|-i}=0)= \textnormal{Pr}(a(i)^{2} < T_{i}).
\end{equation*}
By assumption 1
\begin{equation*}
|a(i)| < |\Delta_{i} + \Gamma_{i,-i}\Gamma_{-i,-i}(J-\Delta)_{-i}| + c_{1}\sum_{k=1}^{M}|(j_{k}-J_{k})|.
\end{equation*}
The term
\begin{equation}
  q=\Delta_{i} + \Gamma_{i,-i}\Gamma_{-i,-i}(J-\Delta)_{-i}
\end{equation}
is normally distributed with mean 0 and variance less than $b_{max}$.
By the proof of lemma \ref{LemmaSSClose}, the term $(j_{k}-J_{k})-v$ is normally distributed with zero mean and variance less than $\sigma_{q}^{2}$ for some where $||v||_{\infty}<\eta(J)$.   It follows then that    

\begin{eqnarray*}
\textnormal{Pr}(a(i)^{2} < T_{i}) &>& \textnormal{Pr}(|\tilde{q}|< \sqrt{T_{i}}-Mc_{1}\eta(J)) \\
&=&\textnormal{erf}\left( \frac{\sqrt{T_{i}}-Mc_{1}\eta(J)}{\sqrt{2(b_{max} + Mc_{1}\sigma_{q}^{2})}}  \right)
\end{eqnarray*}
where $\tilde{q}$ is zero mean normal with variance $(\sqrt{b_{max}} + Mc_{1}\sigma_{q})^{2}$.
It then follows that
\begin{eqnarray*}
  \textnormal{Pr}(z_{i|-i}=0, \forall i>M)&>& \sum_{i=M+1}^{N}\textnormal{erf}\left( \frac{\sqrt{T_{i}}-Mc_{1}\eta(J)}{\sqrt{2(b_{max} + Mc_{1}\sigma_{q}^{2})}} \right) -(N-M-1)
\end{eqnarray*}
\end{proof}

==> bakTable.tex <==
%\usepackage{xcolor,colortbl}
%\usepackage{color}

\definecolor{GrayTable}{gray}{0.85}
\definecolor{LightCyan}{rgb}{.88,1,1}
\definecolor{Pass}{rgb}{0,1,0}
\definecolor{Fail}{rgb}{1,0,0}


\newcolumntype{a}{>{\columncolor{GrayTable}}c}
\newcolumntype{b}{>{\columncolor{white}}c}




\begin{table}
\footnotesize
\centering
\begin{tabular}{|l |l |b | b | b | b|b|}
\hline
\rowcolor{LightCyan}
&  & {KEM} & {KECM} & MCMC & All  & Pairwise  \\
\rowcolor{LightCyan}
$\zeta $      & $\sigma_j^{2}$  &      &      & &Refresh \cite{RefreshTime} & Refresh \cite{VastVolMatrix}\\  
\hline
 $\zeta = 0.999$ & $\sigma_{j}^{2} = 1e-4$ &0.4480e-9 &0.0963e-9  &0.0877e-9 & & \\
 $\zeta = 0.999$& $\sigma_{j}^{2} = 2.5e-5$ &0.1901e-9  & 0.0815e-9 &0.0879e-9 & &\\
 $\zeta = 0.999$& $\sigma_{j}^{2} = 6.25e-6$ &0.1088e-9 &0.0825e-9  &0.0788e-9& & \\
 $\zeta = 0.9995$& $\sigma_{j}^{2} = 1e-4$ &0.1367e-9 &0.0701e-9  &0.0679e-9 & &   \\
 $\zeta = 0.9995$& $\sigma_{j}^{2} = 2.5e-5$ &0.1274e-9  & 0.0798e-9& 0.0889e-9 & &   \\
 $\zeta = 0.9995$& $\sigma_{j}^{2} = 6.25e-6$ &0.089e-9 &0.0804e-9  &0.0892e-9 & &  \\
 $\zeta = 0.9999$& $\sigma_{j}^{2} = 1e-4$ &0.0773e-9 &0.0684e-9&0.0828e-9 & &  \\
 $\zeta = 0.9999$& $\sigma_{j}^{2} = 2.5e-5$ & 0.0876e-9 &0.0780e-9 & 0.0827e-9 & &  \\
 $\zeta = 0.9999$& $\sigma_{j}^{2} = 6.25e-6$ &0.0776e-9 &0.0755e-9  &0.0815e-9 & & \\
 $\zeta = 1$ & N/A &0.0731e-9 &0.0733e-9  &0.0808e-9 \\
 \hline
\end{tabular}
\caption{Numerical results for simulated data for various jump statistics}
\label{TableNumSim_Results}
\end{table} 


\begin{table}
\footnotesize
\centering
\begin{tabular}{|l |l | b | b |}
\hline
\rowcolor{LightCyan}
&  & {KECM} & MCMC   \\
\rowcolor{LightCyan}
$\zeta $      & $\sigma_j^{2}$        &      &\\
\hline

 \hline
\end{tabular}
\caption{Signifcance levels}
\label{TableNumSim_Results_Sig}
\end{table} 


==> robustPCA.tex <==
\section{Relationship with Robust PCA}
Rec

==> secPWEN.tex <==
\section{Pairwise Weighted Elastic Net}

==> tableExample.tex <==
%\usepackage{xcolor,colortbl}
%\usepackage{color}
\newcommand{\mc}[2]{\multicolumn{#1}{c}{#2}}
\definecolor{GrayTable}{gray}{0.85}
\definecolor{LightCyan}{rgb}{.88,1,1}

\newcolumntype{a}{>{\columncolor{GrayTable}}c}
\newcolumntype{b}{>{\columncolor{white}}c}




\begin{table}
\begin{tabular}{l | b | b | b | b}
\hline
\rowcolor{LightCyan}

\mc{1}{}  & \mc{1}{x} & \mc{1}{y} & \mc{1}{w} & \mc{1}{z} \\
\hline
variable 1 & a & b & c & d \\
variable 2 & a & b & c & d \\ \hline
\end{tabular}
\end{table}

==> tableNumSim_Param.tex <==
%\usepackage{xcolor,colortbl}
%\usepackage{color}

\definecolor{GrayTable}{gray}{0.85}


\newcolumntype{a}{>{\columncolor{GrayTable}}c}
\newcolumntype{b}{>{\columncolor{white}}c}




\begin{table}\label{TableNumSim_Param}
\centering
\begin{tabular}{|l | b | b | b | b|}
\hline
\rowcolor{LightCyan}
  & {Value} & {Description} \\
\hline
$\zeta$ & a & 1-probability of a jump  \\
$\sigma_{j}^{2}$ & a & variance of jump  \\
$\sigma_{o}^{2}$ & & variance of observation error\\
\hline
\end{tabular}
\end{table} 
